Deciphering the influence of demographic factors on the treatment of pediatric patients in the emergency department

Persistent demographic disparities have been identified in the treatment of patients seeking care in the emergency department (ED). These may be driven in part by subconscious biases, which providers themselves may struggle to identify. To better understand the operation of these biases, we performed a retrospective cross-sectional analysis using electronic health records describing 339,400 visits to the ED of a single US pediatric medical center between 2019-2024. Odds ratios were calculated using propensity-score matching. Analyses were adjusted for confounding variables, including chief complaint, insurance type, socio-economic deprivation, and patient comorbidities. We also trained a machine learning [ML] model on this dataset to identify predictors of admission. We found significant demographic disparities in admission (Non-Hispanic Black [NHB] relative to Non-Hispanic White [NHW]: OR 0.77, 95\% CI 0.73-0.81; Hispanic relative to NHW: OR 0.80, 95\% CI 0.76-0.83). We also identified disparities in individual decisions taken during the ED stay. For example, NHB patients were significantly less likely than NHW patients to be assigned an `emergent' triage acuity score of (OR 0.70, 95\% CI 0.67-0.72), but emergent NHB patients were also significantly less likely to be admitted than NHW patients with the same triage acuity (OR 0.86, 95\% CI 0.80-0.93). Demographic disparities were particularly acute wherever patients had normal vital signs, public insurance, moderate socio-economic deprivation, or a home address distant from the hospital. An ML model assigned higher importance to triage score for NHB than NHW patients when predicting admission, reflecting these disparities in assignment. We conclude that many visit characteristics, clinical and otherwise, may influence the operation of subconscious biases and affect ML-driven decision support tools.

==> overspill.tex <==
Any additional information about the patient's gender identity was condensed into a single variable indicating whether a patient was transgender or non-binary. Data on patient ethnicity was also available, but due to the large number of possible responses, was not included except where it conflicted with a patient's recorded race. For example, if a patient's race was recorded as Other or Unknown but their ethnicity was Chinese or Hispanic/Latino, their race was `adjusted' to Asian or Hispanic as appropriate. 

e: for example, an infant younger than 28 days is hypotensive if their SBP is lower than 60. We assigned a BP score of 0 if a patient was not hypotensive, and a nonzero score to hypotensive patients corresponding to their distance from the PALS criterion (i.e. to the severity of their hypotension). In this scheme an infant younger than 28 days with an SBP of 58 would have a BP score of 2 (60 - 58).

The propensity score was then simply the fitted `probability' that each visit is from a NHB patient.
